Common-Mode Control and Confinement Inversion of Electrostatically Defined Quantum Dots in a Commercial CMOS Process

Confining electrons or holes in quantum dots formed in the channel of industry-standard fully depleted silicon-on-insulator CMOS structures is a promising approach to scalable qubit architectures. In this article, we present our results on a calibrated model of a commercial nanostructure using the simulation tool Quantum TCAD, along with our experimental verification of all model predictions. We demonstrate here that quantum dots can be formed in the device channel by applying a combination of a common-mode voltage to the source and drain and a back gate voltage. Moreover, in this approach, the amount of quantum dots can be controlled and modified. Also, we report our results on an effective detuning of the energy levels in the quantum dots by varying the barrier gate voltages. Given the need and importance of scaling to larger numbers of qubits, we demonstrate here the feasibility of simulating and improving the design of quantum dot devices before their fabrication based on a commercial process.

==> S05_coulombdiamonds.tex <==
\section{Coulomb Diamond Measurement}

A measurement of Coulomb diamonds was made of the device discussed in the main paper. The measurement results are presented below in Fig.~\ref{fig:nice_diamonds} along with an example calculation of the leverarm extracted using the slopes of two intersecting lines\cite{venkatachalam_local_2012}. The hand calculation shows very close matching with the leverarm predicted by QTCAD simulation ($\approx 0.261~\text{eV/V}$ in simulation, see the main text).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/Supplement/CoulombDiamonds_drawing.png}
    \caption{Charge stability diagram of the quantum dot forming between QA0 and QT0.}
    \label{fig:nice_diamonds}
\end{figure}

The details of the hand calculation to extract the leverarm, which is then scaled by the electron charge $e$.
\begin{align}
    m_{1} &= \frac{\Delta V_{\text{DS}_1}}{\Delta V_{\text{QT0}_1}} \approx \frac{6}{15.7} \approx 0.3822\\
    m_{2} &= \frac{\Delta V_{\text{DS}_2}}{\Delta V_{\text{QT0}_2}} \approx \frac{6}{6.5} \approx 0.9231\\
    \alpha &= \frac{m_{1}m_{2}}{m_{1} + m_{2}} \approx \frac{(0.3822)(0.9231)}{0.3822 + 0.9231} \approx 0.2703 ~\text{V/V}\\
    e\alpha &= 0.2703~\text{eV/V}
\end{align}

An approximate $V_{\text{QT0}}$ distance of $5.4045~\text{mV}$ is measured for the blocked current region to the right of the slopes annotated in Fig.~\ref{fig:nice_diamonds}, denoted $\Delta{V}_{\text{add}}$. This gives a rough indication of the addition energy, $E_{\text{add}}$, of the quantum dot at this filling using the following formula~\cite{kouwenhoven_few-electron_2001}:
\begin{equation}
    E_{\text{add}} = e\alpha\Delta{V}_{\text{add}} \approx (0.2703)(5.4045 \times 10^{-3})~\text{eV/V} \approx 1.4608~\text{meV}
\end{equation}

This is in reasonable agreement with another device with smaller quantum dots in the literature, which results in somewhat higher addition energies ($\approx 5~\text{meV}$)\cite{lim_electrostatically_2009}.

